Synchronization Strings: Efficient and Fast Deterministic Constructions over Small Alphabets

Synchronization strings are recently introduced by Haeupler and Shahrasbi (STOC 2017) in the study of codes for correcting insertion and deletion errors (insdel codes). They showed that for any parameter $\varepsilon>0$, synchronization strings of arbitrary length exist over an alphabet whose size depends only on $\varepsilon$. Specifically, they obtained an alphabet size of $O(\varepsilon^{-4})$, which left an open question on where the minimal size of such alphabets lies between $\Omega(\varepsilon^{-1})$ and $O(\varepsilon^{-4})$. In this work, we partially bridge this gap by providing an improved lower bound of $\Omega(\varepsilon^{-3/2})$, and an improved upper bound of $O(\varepsilon^{-2})$. We also provide fast explicit constructions of synchronization strings over small alphabets. Further, along the lines of previous work on similar combinatorial objects, we study the extremal question of the smallest possible alphabet size over which synchronization strings can exist for some constant $\varepsilon < 1$. We show that one can construct $\varepsilon$-synchronization strings over alphabets of size four while no such string exists over binary alphabets. This reduces the extremal question to whether synchronization strings exist over ternary alphabets.

==> determconstr.tex <==

\section{Deterministic Constructions}
We now construct $\varepsilon$-synchronization strings using synchronization circles. First we recall the following result from  \cite{haeupler2017synchronization}.

\begin{lemma}[Theorem 4.2 of \cite{haeupler2017synchronization}]
\label{insdelCode}
%An $\varepsilon$-synchronization string along with the algorithm in Appendix A form a linear time streaming solution for deletions only $(n,\delta)$-indexing problem guaranteeing $k=\frac{\varepsilon}{1-\varepsilon}n\delta$ misdecodings. Given this, together with an efficient $ECC$ $\mathcal{C}$ over alphabet $\Sigma_C$, that corrects up to $n\delta+2k$ half-errors, one obtains an insertion/deletion code that can be decoded from up to $n\delta$ deletions.
Given an $\varepsilon$-synchronization string $S$ with length $n$, alphabet $\Sigma_S$, and an efficient ECC $\mathcal{C}$ with block length $n$, alphabet $\Sigma_C$, that corrects up to $n\delta \frac{1+\varepsilon}{1-\varepsilon}$ half-errors, one can obtain an insertion/deletion code $\mathcal{C}'$  that can be decoded from up to $n\delta$ deletions, where $ \mathcal{C}' = \{(c'_1, \ldots, c'_n)| \forall  i\in [n],  c'_i = (c_i, S[i]), (c_1,\ldots, c_n) \in \mathcal{C}  \} $.

\end{lemma}
Using the insertion deletion code in this lemma, we have the following construction of a synchronization circle $S$ of length $n$.


\begin{algo}
\label{algo}
Main Construction.

For every $n, m \in \mathbb{N}, m\leq n$, we have the following.

\textbf{Input:}
\begin{enumerate}
  \item A ECC $\tilde{\mathcal{C}}\subset\Sigma_{\tilde{c}}^m$, with distance $ \delta m $ and $|\tilde{\mathcal{C}}| \geq \ell = \lceil \frac{n}{m}\rceil$.
  \item An $\varepsilon$-synchronization circle $SC$ of length $m$ over alphabet $\Sigma_{sc}$ i.e. $ SC=(sc_1,sc_2,\dots,sc_m) \in\Sigma_{sc}^m$.
\end{enumerate}

\textbf{Output:} An $ \varepsilon'$-synchronization  $S$ circle of length $n$.

\textbf{Operations:}

\begin{itemize}
  \item Construct a new code $\mathcal{C}\subset\Sigma^m$ s.t.
$$ \mathcal{C} = \{c=((\tilde{c}_1,sc_1),(\tilde{c}_2,sc_2),\dots,(\tilde{c}_m,sc_m))|(\tilde{c}_1,\tilde{c}_2,\dots,\tilde{c}_m)\in\tilde{\mathcal{C}}\},$$
where $\Sigma=\Sigma_{\tilde{c}}\times\Sigma_{sc}$.
  \item Choose $\ell $ codewords $C_1,C_2,\dots,C_{\ell}$ from $\mathcal{C}$.
  \item Let $S$ be concatenation of these codewords: $S=C_1\circ C_2\circ\dots\circ C_{\ell}$.
\end{itemize}

\end{algo}

\begin{lemma}
\label{mainlemmaofalgo}
The output $S$ in Algorithm \ref{algo} is an $\varepsilon'$-synchronization circle, where $\varepsilon' \leq 10(1-\frac{1-\varepsilon}{1+\varepsilon}\delta) $.
\end{lemma}

\begin{proof}
Suppose $\tilde{\mathcal{C}}$ can correct up to $\delta m$ half-errors. Then according to lemma \ref{insdelCode}, $\mathcal{C}$ can correct up to $\frac{1-\varepsilon}{1+\varepsilon} \delta m$ deletions.

Let $\alpha=1-\frac{1-\varepsilon}{1+\varepsilon}\delta$. Notice that $\mathcal{C}$ has the following properties:
\begin{enumerate}
  \item $LCS(\mathcal{C}) = \max_{c_1, c_2\in C}{LCS(c_1, c_2)} \leq \alpha m$
  \item Each codeword in $\mathcal{C}$ is an $\varepsilon$-synchronization circle over $\Sigma$.
\end{enumerate}

Consider any shift of the start point of $S$, we only need to prove that $\forall 1\leq i < j < k\leq n, LCS(S[i,j],S[j+1,k])<\frac{\varepsilon'}{2}(k-i)$. First we prove the lemma below.

\begin{lemma}
\label{lcs}
Suppose $T_1$ is the concatenation of $\ell_1$ strings, $T_1=S_1\circ\dots\circ S_{\ell_1}$ and $T_2$ is the concatenation of $\ell_2$ strings, $T_2=S'_1\circ\dots\circ S'_{\ell_2}$. If  there exists an integer $t$ such that for all $i, j$, we have $LCS(S_i, S'_j) \leq t$, then we have $LCS(T_1, T_2) \leq (\ell_1+\ell_2)t$.
%Suppose $T_1$ and $T_2$ are concatenations of different codewords from $\mathcal{C}$, where all the codewords used are from $\mathcal{C}$ and different. Then $LCS(T_1,T_2)\leq (\ell_1+\ell_2)\alpha m$.
\end{lemma}
\begin{proofofnobox}[Lemma \ref{lcs}]
We rename the strings in $T_1$ by $S_1, \cdots, S_{\ell_1}$ and rename the strings in $T_2$ by $S_{\ell_1+1}, \cdots, S_{\ell_1+\ell_2}$. Suppose the longest common subsequence between $T_1$ and $T_2$ is $\tilde{T}$, which can be viewed as a matching between $T_1$ and $T_2$.
%Suppose in this match, the $i$th codeword $C_i$ in $S_1$ matches to a (consecutive) substring $T_i$ in $S_2$ of length $j_i$.


we can divide $\tilde{T}$ sequentially into disjoint intervals, where each
interval corresponds to a common subsequence between a different pair
of strings $(S_i, S_j)$, where $S_i$ is from $T_1$ and $S_j$ is from $T_2$. In
addition, if we look at the intervals from left to right, then for any
two consecutive intervals and their corresponding pairs $(S_i, S_j)$ and $(S_{i'}, S_{j'})$, we must have $i' \geq i$ and $j' \geq j$  since the matchings which correspond to two intervals cannot cross each other. Furthermore either $i' > i$
or $j' > j$ as the pair $(S_i, S_j)$ is different from $(S_{i'}, S_{j'})$. 

Thus, starting from the first interval, we can
label each interval with either $i$ or $j $ such that every interval
receives a different label, as follows. We label the first interval using either $i$ or $j$. Then, assuming we have already labeled some intervals and now look at the next interval. Without loss of generality assume that the previous interval is labeled using $i$, now if the current $i' > i$ then we can label the current interval using $i'$; otherwise we must have $j'>j$ so we can label the current interval using $j'$. Thus the total number of the labels is at
most $l_1+l_2$, which means the total number of the intervals is also at
most $l_1+l_2$. Note that each interval has length at most $t$, therefore we can upper bound $LCS(T_1, T_2)$ by
 $(l_1+l_2)t$.


%
%For this match, we denote $T_i$ as the shortest (continuous) substring in $S_2$ which $C_i$ matches to. Let $j_i = |T_i|$.
%See Figure \ref{1} as an example in which  $j_1=3,j_2=5,j_3=4$.
%\begin{figure}[H]
%  \centering
%  \includegraphics[width=8cm]{LCS.png}\\
%  \caption{Example of match between $S_1$ and $S_2$}\label{1}
%\end{figure}
%
%Notice that $\sum_{i=1}^{\ell_1}j_i\leq \ell_2 m$. The number of codewords that intersect with
%%the continuous substring matching with $C_i$
%$T_i$
%is at most $\lceil\frac{j_i}{m}\rceil+1$. Thus the length of the common subsequence $i$th codeword matches to is at most $(\lceil\frac{j_i}{m}\rceil+1)\alpha m$. Hence we have
%\begin{align*}
%LCS(S_1,S_2)&\leq \sum_{i=1}^{\ell_1}(\lceil\frac{j_i}{m}\rceil+1)\alpha m\\
%&\leq \sum_{i=1}^{\ell_1} (\frac{j_i}{m}+2)\alpha m\\
%&= \sum_{i=1}^{\ell_1} j_i\alpha +2\sum_{i=1}^{\ell_1}\alpha m\\
%&\leq(\ell_2+2\ell_1)\alpha m
%\end{align*}
%Thus $LCS(S_1,S_2)$ is at most $(\ell_2+2\ell_1)\alpha m.\square$

\end{proofofnobox}

Suppose $S_1=S[i,j]$ and $S_2=S[j+1,k]$. Let $\varepsilon' = 10\alpha$.
\paragraph{Case 1:} $k-i>m$. Let $|S_1|=s_1$ and $|S_2|=s_2$, thus $s_1+s_2 > m$. If we look at each $S_h$ for $h=1, 2$, then $S_h$ can be divided into some consecutive codewords, plus at most two incomplete codewords at both ends. In this sense each $S_h$ is the concatenation of $\ell_h$ strings with $\ell_h < \frac{s_h}{m}+2$. An example of the worst case appears in Figure \ref{4}.

\begin{figure}[H]
  \centering
  \includegraphics[width=8cm]{case2_0.png}\\
  \caption{Example of the worst case, where $j$ splits a codeword, and there are two incomplete codewords at both ends.}\label{4}
\end{figure}

Now consider the longest common subsequence between any pair of these strings where one is from $S_1$ and the other is from $S_2$, we claim that the length of any such longest common subsequence is at most $\alpha m$. Indeed, if the pair of strings are from two different codewords, then by the property of the code $\mathcal{C}$ we know the length is at most $\alpha m$. On the other hand, if the pair of strings are from a single codeword (this happens when $j$ splits a codeword, or when $S[i]$ and $S[k]$ are in the same codeword), then they must be two disjoint intervals within a codeword. In this case, by the property that any codeword is also a synchronization circle, the length of the longest common subsequence of this pair is at most $\frac{\varepsilon}{2} m$.

Note that $\alpha=1-\frac{1-\varepsilon}{1+\varepsilon}\delta \geq  1-\frac{1-\varepsilon}{1+\varepsilon} =\frac{2\varepsilon}{1+\varepsilon} \geq \varepsilon$ (since $\delta, \varepsilon \in (0, 1)$). Thus $\frac{\varepsilon}{2} m < \alpha m$. Therefore, by Lemma~\ref{lcs}, we have 

\begin{align*}
& LCS(S_1, S_2) \\ 
< &(\frac{s_1}{m}+2+\frac{s_2}{m}+2) \alpha m \\
= &\alpha (s_1+s_2+4 m) \\
< & 5 \alpha (s_1+s_2) \\
= & 5 \alpha (k-i) = \frac{\varepsilon'}{2}(k-i)
\end{align*}

\iffalse
If $k-i>m,m|j$, then $S[j]$ is exactly the last symbol of a codeword. Let $\ell_1$ and $\ell_2$ be the number of complete codewords in $S_1$ and $S_2$. If $\ell_1+\ell_2=0$, which means that there is no complete codeword in either $S_1$ or $S_2$, then $LCS(S_1,S_2)\leq\alpha m<\alpha (k-i)<\frac{\varepsilon'}{2}(k-i)$. See the example in Figure \ref{2}.

\begin{figure}[H]
  \centering
  \includegraphics[width=8cm]{case1_0.png}\\
  \caption{Example in which $k-i>m, m|j$ and $\ell_1+\ell_2=0$}\label{2}
\end{figure}

Now assume that $\ell_1+\ell_2\geq 1$. Except for the complete codewords, there may be an incomplete codeword $C_{head}=S[i,j-\ell_1 m]$ in $S_1$ and $C_{tail}=S[j+\ell_2 m+1,k]$ in $S_2$. As shown in Figure \ref{3}. In this case, we can extend both $C_{head}$ and $C_{tail}$ into complete codewords, and the length of the longest common subsequence between $S_1$ and $S_2$ cannot decrease. Now we have at most $l_1+1$ complete codewords in $S_1$ and $l_2+1$ complete codewords in $S_2$.

\begin{figure}[H]
  \centering
  \includegraphics[width=8cm]{case1_1.png}\\
  \caption{Example in which $k-i>m, m|j, \ell_1=0, \ell_2=1$}\label{3}
\end{figure}

Thus we have
\begin{align*}
&LCS(S_1,S_2)\\
\leq & LCS(C_{head},S[j+1,j+\ell_2 m])+LCS(S[j-\ell_1 m, j],S[j+1,j+\ell_2 m])+LCS(S[j-\ell_1 m, j],C_{tail})\\
\leq & (\ell_2+1)\alpha m+(\ell_1+\ell_2)\alpha m+ (\ell_1+1)\alpha m\\
\leq & (2\ell_2+2\ell_1+2)\alpha m\\
\leq & 4(\ell_1+\ell_2)\alpha m\\
\leq &4\alpha(k-i)<\frac{\varepsilon'}{2}(k-i)
\end{align*}

\paragraph{Case 2:} If $k-i>m,m\nmid j$, then $S[j]$ splits a codeword, which we denote as $C_0$. Suppose the part in $S_1$ is $C_0^1$  and that in $S_2$ is $C_0^2$. Notice that $LCS(C_0^1,C_0^2)\leq \frac{\varepsilon}{2} m$, according to the property of synchronization circle. Similar to Case 1, let $\ell_1$ and $\ell_2$ be the number of complete codewords in $S_1$ and $S_2$. Moreover, denote the substring in $S_1$ before $C_0^1$ as $C_{head}$, and the substring in $S_2$ after $C_0^2$ as $C_{tail}$. If $\ell_1+\ell_2=0$, then 
\begin{align*}
& LCS(S_1,S_2)\\
\leq & LCS(C_{head}, C_0^2)+  LCS(C_{head},C_{tail})  +  LCS(C_0^1,C_0^2) + LCS(C_0^1, C_{tail})\\
\leq & \alpha m + \alpha m  + \frac{\varepsilon}{2}m + \alpha m = 3\alpha m +\frac{\varepsilon}{2} m
\end{align*} 
 
Notice that for $\varepsilon\in (0,1)$, $\frac{1-\varepsilon}{1+\varepsilon}+\varepsilon = \frac{1+\varepsilon^2}{1+\varepsilon} < 1$, which means $\frac{\varepsilon}{2} < \varepsilon < 1-\frac{1-\varepsilon}{1+\varepsilon} < 1-\frac{1-\varepsilon}{1+\varepsilon}\delta = \alpha$. So $LCS(C_0^1,C_0^2)\leq \frac{\varepsilon}{2}m \leq \alpha m$. Thus $LCS(S_1, S_2) \leq 3\alpha m +\frac{\varepsilon}{2} m \leq 4\alpha m \leq \frac{\varepsilon'}{2} (k-i)$. As in Figure \ref{4}.


Now assume that $\ell_1+\ell_2\geq 1$. We denote the substring of $S_1$ from the first symbol to the beginning of $C_0^1$ as $S_1'$ and the substring of $S_2$ from the end of $C_0^2$ to the end as $S_2'$. If the longest common subsequence contains a match between $C_0^1$ and $C_0^2$, e.g. in figure \ref{5}, then we have
\begin{align*}
&LCS(S_1,S_2)\\
\leq &LCS(C_0^1,C_0^2)+LCS(C_0^1,S_2')+LCS(S_1', C_0^2) + LCS(S_1', S_2')\\
\leq &\alpha m + (\ell_2+1)\alpha m + (\ell_1+1)\alpha m + (l_1 + l_2 + 2) \alpha m\\
\leq &(2\ell_1+2\ell_2+5)\alpha m\\
\leq &7(\ell_1+\ell_2)\alpha m\\
\leq &7\alpha(k-i)<\frac{\varepsilon'}{2}(k-i),
\end{align*}
where the first inequality is by Lemma \ref{lcs}.

\begin{figure}[H]
  \centering
  \includegraphics[width=10cm]{case2_10.png}\\
  \caption{Example in which there's match between $c_0^1$ and $c_0^2$}\label{5}
\end{figure}

If there's no match between $C_0^1$ and $C_0^2$ in the longest common subsequence, then the problem becomes similar to case1, as in figure \ref{6}. We have that:
\begin{align*}
&LCS(S_1,S_2)\\
\leq &LCS(S_1',C_0^2)+LCS(S_1',S_2')+LCS(C_0^1,S_2)\\
\leq &(\ell_1+1)\alpha m+(2\ell_2+3\ell_1+2)\alpha m +(\ell_2+1)\alpha m\\
\leq &8(\ell_1+\ell_2)\alpha m\\
\leq &8\alpha(k-i)\leq \frac{\varepsilon'}{2}(k-i)
\end{align*}
\begin{figure}[H]
  \centering
  \includegraphics[width=8cm]{case2_11.png}\\
  \caption{Example in which there's no match between $c_0^1$ and $c_0^2$}\label{6}
\end{figure}
\fi
\paragraph{Case 2:} If $k-i\leq m$, then according to the property of synchronization circle $ SC $, we know that the longest common subsequence of $S_1$ and $S_2$ is less than $\frac{\varepsilon}{2}(k-i)\leq \alpha(k-i)\leq\frac{\varepsilon'}{2}(k-i)$.

As a result, the longest common subsequence of $S[i,j]$ and $S[j+1,k]$ is less than $\frac{\varepsilon'}{2}(k-i)$, which means that $S$ is an $\varepsilon'$-synchronization circle. %string. It is  an $\varepsilon'$-synchronization circle since the analysis still holds when the interval from $i$ to $k$ crosses the end of the string.
\end{proof}


\begin{lemma}
\label{smallcode}

For any $n\in \mathbb{N}$, any $\varepsilon \in [0,1]$,
one can construct a ECC in time $  O(2^{\varepsilon n} (\frac{2e}{\varepsilon})^n n \log(1/\varepsilon))  $ and space $  O(2^{\varepsilon n} n \log (1/\varepsilon) ) $, with block length $n$, number of codewords $  2^{\varepsilon n}$, distance $ d = (1-\varepsilon)n$, alphabet size $2e/\varepsilon$.
\end{lemma}

\begin{proof}

We conduct a brute-force search here to find all the codewords one by one.

We denote the code as $\mathcal{C}$ and the alphabet as $\Sigma$. Let $|\Sigma| = q$.
At first, let $\mathcal{C} = \emptyset$. Then we add an arbitrary element in $\Sigma^n$ to $\mathcal{C}$. Every time after a new element $C$ is added to $\mathcal{C}$, we exclude every such element in $\Sigma^{n}$ that has distance less than $d$ from $C$. Then we pick an arbitrary one from the remaining elements, adding it to $\mathcal{C}$. Keep doing this until $|\mathcal{C}| = 2^{\varepsilon n}$.

Note that given $C \in \Sigma^n$, the total number of elements that have distance less than $d$ to $C$, is at most ${n \choose d} q^d  = {n \choose (n-d)} q^d \leq (\frac{e}{\varepsilon})^{\varepsilon n} q^{(1-\varepsilon) n} $. We have to require that  $ |\mathcal{C}| (\frac{e}{\varepsilon})^{\varepsilon n} q^{(1-\varepsilon) n} \leq q^n $.
Let $q = 2e/\varepsilon$. So $\mathcal{C}$ can be $2^{\varepsilon n}$.

The exclusion operation takes time $  O((\frac{2e}{\varepsilon})^n n \log(1/\varepsilon)) $ as we have to
exhaustively search the space and for each word we have to compute it's hamming distance to the new added code word. Since there are  $  2^{\varepsilon n}$ code words, the time complexity is as stated.

We have to record those code words, so the space complexity is also as stated.
\end{proof}


\begin{theorem}
\label{mainTheorem}
For  any $n\in \mathbb{N}$ and any $\varepsilon \in (0, 1)$, an $\varepsilon$-synchronization circle $S$ of length $n$ over alphabet $\Sigma$ where $|\Sigma| = O(\varepsilon^{-3})$ can be constructed in time  $(O(\frac{1}{\varepsilon^2}))^{O(\frac{\log n}{\varepsilon})}\cdot \poly (\frac{\log n}{\varepsilon})$.  If $\varepsilon$ is a constant, then the running time is $\poly(n)$.
\end{theorem}
\begin{proof}
By Lemma \ref{smallcode}, we can construct a  ECC $ \mathcal{C} $ with block length $m = O(\frac{\log n}{\varepsilon})$, $|\mathcal{C}  | = n$, distance $\rho m$,  $\rho=\frac{1+\frac{\varepsilon}{30}}{1-\frac{\varepsilon}{30}}(1-\frac{\varepsilon}{10})=1-\Omega(\varepsilon)$,  alphabet $\Sigma_{ \mathcal{C} }$ of size $O(1/\varepsilon)$. Let $\mathcal{SC}$ be an $\frac{\varepsilon}{30}$-synchronization circle over alphabet $\Sigma_{sc}$ with length $m$. Let $|\Sigma_{sc}| = O(\varepsilon^{-2})$. Then according to the construction algorithm and lemma \ref{mainlemaofalgo1}, we have an $\varepsilon$-synchronization string $S$.

The construction of  $ SC $ takes $(O(\frac{1}{\varepsilon^2}))^{O(m)}\cdot \poly (m)=(O(\frac{1}{\varepsilon^2}))^{O(\frac{\log n}{\varepsilon})}\cdot \poly (\frac{\log n}{\varepsilon})$. By Lemma \ref{smallcode}, constructing $\mathcal{C}$ takes time $ O(2^{\varepsilon m} (\frac{2e}{\varepsilon})^m m \log(1/\varepsilon))  $. Thus the total running time is $(O(\frac{1}{\varepsilon^2}))^{O(\frac{\log n}{\varepsilon})}\cdot \poly (\frac{\log n}{\varepsilon})$. Regarding $\varepsilon$ as a constant, it is $\poly(n)$.
\end{proof}


To make the construction more efficient, we can use a 2-level recursion to reduce the running time to $n\cdot \poly\log n$, which is near linear.

\begin{theorem}
\label{efficient}
There exists a constant $C>1$ such that for any $n\in \mathbb{N}$ and any $\varepsilon \geq \frac{C (\log \log n)^2}{\log n}$, an $\varepsilon$-synchronization circle $S$ over alphabet $\Sigma$ where $|\Sigma| = O(\varepsilon^{-4})$ can be constructed in $O(n\cdot  (\log \log n)^2)$ time.
\end{theorem}

\begin{proof}
First by Theorem \ref{mainTheorem} we can construct a synchronization circle $S_0$ of length $m' = O(\frac{\log n (\log \log n + \log \frac{1}{\varepsilon}) }{\varepsilon^2} )$ over alphabet $\Sigma_0$ of size $O(\varepsilon^{-3})$. Let $ECC$ $\mathcal{C}$ be the concatenation code of two codes, an outer $(m=O(\frac{\log n}{\varepsilon}),  \Omega(\varepsilon m) , (1-O(\varepsilon))m)$ Reed-Solomon code with alphabet size $m$, and an inner code by Lemma \ref{smallcode} with block length $m_0 = O(\frac{\log m}{\varepsilon})$, number of codewords $m$, distance $(1-O(\varepsilon))m_0$,  alphabet size $O(1/\varepsilon)$. Thus $\mathcal{C}$ is an ECC with block length $m' =m m_0$, number of code words at least $n$, distance  $(1-O(\varepsilon))m'$, alphabet size $O(1/\varepsilon)$. Then one can use $S_0$ together with $\mathcal{C}$ to construct an $\varepsilon$-synchronization string over alphabet $\Sigma$ of size $O(\varepsilon^{-4})$, according to Algorithm \ref{algo}.

By Theorem \ref{mainTheorem}, the construction of $S_0$ takes $(O(  \frac{1}{\varepsilon^2} ))^{O(\frac{\log m'}{\varepsilon})}\cdot \poly (\frac{\log m'}{\varepsilon})$. The time to copy it for $n$ positions is $O(n \log(1/\varepsilon))$. The time to compute the inner code is $m(\frac{2e}{\varepsilon})^{O(m_0)} O(m_0 \log \frac{1}{\varepsilon})$. The inner code only have to be computed once. Computing the outer Reed-Solomon code takes time $O(m \log^3 m)$ by Theorem \ref{RSenctime}.
Copying the inner code for all symbols of one
outer codeword takes time $O(m m_0 \log(1/\varepsilon))$, so the total
time to compute one codeword of the concatenated code is $O(m \log^3m+ m m_0 \log(1/\varepsilon))$. We use $n/m'=n/(m m_0)$ concatenated codewords for  $S$, so this takes time
$\frac{n}{m m_0}(O(m \log^3m+ m m_0 \log(1/\varepsilon)))$.
Thus the total running time is
%$$\frac{\varepsilon\log n}{\log\log n}O(\frac{1}{\varepsilon})^{O(\frac{\log\log n}{\varepsilon})}+ O(\frac{n}{m} m \cdot \poly \log m  + m(\frac{1}{\varepsilon})^{O(m_0)}).$$
\begin{equation}
\begin{split}
&(O(  \frac{1}{\varepsilon^2}))^{O(\frac{\log m'}{\varepsilon})}\cdot \poly (\frac{\log m'}{\varepsilon}) + O(n \log(1/\varepsilon)) \\
+ & m(\frac{2e}{\varepsilon})^{O(m_0)} O(m_0 \log \frac{1}{\varepsilon})
 +  \frac{n}{m_0}( O( \log^3 m+ m_0 \log(1/\varepsilon)))\\
= &  (O(\frac{1}{\varepsilon}))^{O(\frac{\log \log n+\log(1/\varepsilon)}{\varepsilon})}+O(n \log(1/\varepsilon))+ O(\varepsilon n  \log^2 \frac{\log n}{\varepsilon}).
\end{split}
\end{equation}


Thus as long as $\varepsilon \geq \frac{C (\log \log n)^2}{\log n}$ for some constant $C>1$,  the running time is then $O(n\cdot  (\log \log n)^2)$, which is near linear.


%
%First we use same technique in Theorem \ref{mainTheorem} to construct a synchronization string $\mathcal{S}_0$, which is also a synchronization circle, of length $m=O(\log n)$ over alphabet $\Sigma_0$ of size $O(\varepsilon^{-3})$. Let $ECC$ $\mathcal{C}$ be a concatenation code of two Reed-Solomon code, an outer code $[n_1,k_1,d_1]_q$ and and inner code $[n_2,k_2,d_2]_q$ where $q=O(\frac{1}{\varepsilon})$. Then one can use $\mathcal{S}_0$ together with $\mathcal{C}$ to construct an $\varepsilon$-synchronization string over alphabet $\Sigma$ of size $O(\varepsilon^{-4})$.
%
%The construction of $\mathcal{S}_0$ takes $\frac{\varepsilon\log n}{\log\log n}O(\frac{1}{\varepsilon})^{O(\frac{\log\log n}{\varepsilon})}$. The time to computer the inner code is $\frac{\varepsilon\log n}{\log\log n}O(\frac{1}{\varepsilon})^{O(\frac{\log\log n-\log(\varepsilon)}{\varepsilon})}$. Later when computing outer codeword and encode each symbol, we only need to copy the inner code. As we need $\frac{n}{n_1n_2}$ codewords, the time for copying the inner codeword is $\frac{n}{n_1n_2}\cdot O(n_1\poly\log (n_1)\cdot(n_2\log (\frac{1}{\varepsilon})))$. Thus the total running time is $\frac{\log n}{\log\log n}O(\frac{1}{\varepsilon})^{O(\frac{\log\log n+\log(1/\varepsilon)}{\varepsilon})}+O(n\cdot \poly(\log\log n+\log(1/\varepsilon)))$. Regarding $\varepsilon$ as a constant, the running time is then $n \poly(\log\log n)$, which is near linear.
\end{proof}
